On effects of Knowledge Distillation on Transfer Learning

Knowledge distillation is a popular machine learning technique that aims to transfer knowledge from a large 'teacher' network to a smaller 'student' network and improve the student's performance by training it to emulate the teacher. In recent years, there has been significant progress in novel distillation techniques that push performance frontiers across multiple problems and benchmarks. Most of the reported work focuses on achieving state-of-the-art results on the specific problem. However, there has been a significant gap in understanding the process and how it behaves under certain training scenarios. Similarly, transfer learning (TL) is an effective technique in training neural networks on a limited dataset faster by reusing representations learned from a different but related problem. Despite its effectiveness and popularity, there has not been much exploration of knowledge distillation on transfer learning. In this thesis, we propose a machine learning architecture we call TL+KD that combines knowledge distillation with transfer learning; we then present a quantitative and qualitative comparison of TL+KD with TL in the domain of image classification. Through this work, we show that using guidance and knowledge from a larger teacher network during fine-tuning, we can improve the student network to achieve better validation performances like accuracy. We characterize the improvement in the validation performance of the model using a variety of metrics beyond just accuracy scores, and study its performance in scenarios such as input degradation.

==> abbrs.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l p{5in}}
  NN & Neural Network\\
  DL & Deep Learning\\
  TL & Transfer Learning\\
  KD & Knowledge Distillation\\
  TL+KD & Transfer Learning with Knowledge Distillation\\
  CIFAR & Canadian Institute for Advanced Research\\
  ILSVRC & ImageNet Large Scale Visual Recognition Challenge\\
  SGD & Stochastic Gradient Descent \\
  LR & Learning Rate\\
  ANN & Artificial Neural Network\\
  CNN & Convolutional Neural Network\\
  RNN & Recurrent Neural Network\\
  ViT & Vision Transformers\\
  $\mathbf{x}$    & Truth value x\\
  $\tilde{\mathbf{x}}$    & Measured value x\\
  $\hat{\mathbf{x}}$    & Estimated or computed value x\\
\end{tabular*}


==> chapters/ack.tex <==
----

==> chapters/app_model.tex <==
\subsection{ResNet18}
Resnet18 network used as Student network whose last layer has been modified to output 10 classes for the CIFAR10 dataset instead of 1000 classes for ImageNet is described below.   

\begin{Verbatim}[frame=single]
----------------------------------------------------------------
        Layer (type)               Output Shape         Param #
================================================================
            Conv2d-1         [-1, 64, 112, 112]           9,408
       BatchNorm2d-2         [-1, 64, 112, 112]             128
              ReLU-3         [-1, 64, 112, 112]               0
         MaxPool2d-4           [-1, 64, 56, 56]               0
            Conv2d-5           [-1, 64, 56, 56]          36,864
       BatchNorm2d-6           [-1, 64, 56, 56]             128
              ReLU-7           [-1, 64, 56, 56]               0
            Conv2d-8           [-1, 64, 56, 56]          36,864
       BatchNorm2d-9           [-1, 64, 56, 56]             128
             ReLU-10           [-1, 64, 56, 56]               0
       BasicBlock-11           [-1, 64, 56, 56]               0
           Conv2d-12           [-1, 64, 56, 56]          36,864
      BatchNorm2d-13           [-1, 64, 56, 56]             128
             ReLU-14           [-1, 64, 56, 56]               0
           Conv2d-15           [-1, 64, 56, 56]          36,864
      BatchNorm2d-16           [-1, 64, 56, 56]             128
             ReLU-17           [-1, 64, 56, 56]               0
       BasicBlock-18           [-1, 64, 56, 56]               0
           Conv2d-19          [-1, 128, 28, 28]          73,728
      BatchNorm2d-20          [-1, 128, 28, 28]             256
             ReLU-21          [-1, 128, 28, 28]               0
           Conv2d-22          [-1, 128, 28, 28]         147,456
      BatchNorm2d-23          [-1, 128, 28, 28]             256
           Conv2d-24          [-1, 128, 28, 28]           8,192
      BatchNorm2d-25          [-1, 128, 28, 28]             256
             ReLU-26          [-1, 128, 28, 28]               0
       BasicBlock-27          [-1, 128, 28, 28]               0
           Conv2d-28          [-1, 128, 28, 28]         147,456
      BatchNorm2d-29          [-1, 128, 28, 28]             256
             ReLU-30          [-1, 128, 28, 28]               0
           Conv2d-31          [-1, 128, 28, 28]         147,456
      BatchNorm2d-32          [-1, 128, 28, 28]             256
             ReLU-33          [-1, 128, 28, 28]               0
       BasicBlock-34          [-1, 128, 28, 28]               0
           Conv2d-35          [-1, 256, 14, 14]         294,912
      BatchNorm2d-36          [-1, 256, 14, 14]             512
             ReLU-37          [-1, 256, 14, 14]               0
           Conv2d-38          [-1, 256, 14, 14]         589,824
      BatchNorm2d-39          [-1, 256, 14, 14]             512
           Conv2d-40          [-1, 256, 14, 14]          32,768
      BatchNorm2d-41          [-1, 256, 14, 14]             512
             ReLU-42          [-1, 256, 14, 14]               0
       BasicBlock-43          [-1, 256, 14, 14]               0
           Conv2d-44          [-1, 256, 14, 14]         589,824
      BatchNorm2d-45          [-1, 256, 14, 14]             512
             ReLU-46          [-1, 256, 14, 14]               0
           Conv2d-47          [-1, 256, 14, 14]         589,824
      BatchNorm2d-48          [-1, 256, 14, 14]             512
             ReLU-49          [-1, 256, 14, 14]               0
       BasicBlock-50          [-1, 256, 14, 14]               0
           Conv2d-51            [-1, 512, 7, 7]       1,179,648
      BatchNorm2d-52            [-1, 512, 7, 7]           1,024
             ReLU-53            [-1, 512, 7, 7]               0
           Conv2d-54            [-1, 512, 7, 7]       2,359,296
      BatchNorm2d-55            [-1, 512, 7, 7]           1,024
           Conv2d-56            [-1, 512, 7, 7]         131,072
      BatchNorm2d-57            [-1, 512, 7, 7]           1,024
             ReLU-58            [-1, 512, 7, 7]               0
       BasicBlock-59            [-1, 512, 7, 7]               0
           Conv2d-60            [-1, 512, 7, 7]       2,359,296
      BatchNorm2d-61            [-1, 512, 7, 7]           1,024
             ReLU-62            [-1, 512, 7, 7]               0
           Conv2d-63            [-1, 512, 7, 7]       2,359,296
      BatchNorm2d-64            [-1, 512, 7, 7]           1,024
             ReLU-65            [-1, 512, 7, 7]               0
       BasicBlock-66            [-1, 512, 7, 7]               0
AdaptiveAvgPool2d-67            [-1, 512, 1, 1]               0
           Linear-68                   [-1, 10]           5,130
================================================================
% Input size (MB): 0.57
% Forward/backward pass size (MB): 62.79
% Params size (MB): 42.65
% Estimated Total Size (MB): 106.01
% ----------------------------------------------------------------
\end{Verbatim}


\subsection{ViT}
ViT B\_16 network used as Teacher network whose last layer has also been modified to output 10 classes for CIFAR10 dataset instead of 1000 classes for ImageNet is described below.  

\begin{Verbatim}[frame=single]

______________________________________________________________
 Layer (type)                   Output Shape         Param #  
==============================================================
 input_3 (InputLayer)           [(None, 32, 32, 3)]  0        
 data_augmentation (Sequential)  (None, 72, 72, 3)   7        
 patches_1 (Patches)            (None, None, 108)    0        
 patch_encoder_1 (PatchEncoder)  (None, 144, 64)     16192    
 layer_normalization_17 (LN)     (None, 144, 64)     128      
 multi_head_attention_8 (MH)     (None, 144, 64)     66368    
 add_16 (Add)                   (None, 144, 64)      0        
 layer_normalization_18 (LN)     (None, 144, 64)     128      
 dense_21 (Dense)               (None, 144, 128)     8320     
 dropout_19 (Dropout)           (None, 144, 128)     0        
 dense_22 (Dense)               (None, 144, 64)      8256     
 dropout_20 (Dropout)           (None, 144, 64)      0        
 add_17 (Add)                   (None, 144, 64)      0        
 layer_normalization_19 (LN)     (None, 144, 64)     128      
 multi_head_attention_9 (MH)     (None, 144, 64)     66368    
 add_18 (Add)                   (None, 144, 64)      0        
 layer_normalization_20 (LN)     (None, 144, 64)     128      
 dense_23 (Dense)               (None, 144, 128)     8320     
 dropout_21 (Dropout)           (None, 144, 128)     0        
 dense_24 (Dense)               (None, 144, 64)      8256     
 dropout_22 (Dropout)           (None, 144, 64)      0        
 add_19 (Add)                   (None, 144, 64)      0        
 layer_normalization_21 (LN)     (None, 144, 64)     128      
 multi_head_attention_10 (MH)    (None, 144, 64)     66368    
 add_20 (Add)                   (None, 144, 64)      0        
 layer_normalization_22 (LN)     (None, 144, 64)     128      
 dense_25 (Dense)               (None, 144, 128)     8320     
 dropout_23 (Dropout)           (None, 144, 128)     0        
 dense_26 (Dense)               (None, 144, 64)      8256     
 dropout_24 (Dropout)           (None, 144, 64)      0        
 add_21 (Add)                   (None, 144, 64)      0        
 layer_normalization_23 (LN)     (None, 144, 64)     128      
 multi_head_attention_11 (MH)    (None, 144, 64)     66368    
 add_22 (Add)                   (None, 144, 64)      0        
 layer_normalization_24 (LN)     (None, 144, 64)     128      
 dense_27 (Dense)               (None, 144, 128)     8320     
 dropout_25 (Dropout)           (None, 144, 128)     0        
 dense_28 (Dense)               (None, 144, 64)      8256     
 dropout_26 (Dropout)           (None, 144, 64)      0        
 add_23 (Add)                   (None, 144, 64)      0        
 layer_normalization_25 (LN)     (None, 144, 64)     128      
 multi_head_attention_12 (MH)    (None, 144, 64)     66368    
 add_24 (Add)                   (None, 144, 64)      0        
 layer_normalization_26 (LN)     (None, 144, 64)     128      
 dense_29 (Dense)               (None, 144, 128)     8320     
 dropout_27 (Dropout)           (None, 144, 128)     0        
 dense_30 (Dense)               (None, 144, 64)      8256     
 dropout_28 (Dropout)           (None, 144, 64)      0        
 add_25 (Add)                   (None, 144, 64)      0        
 layer_normalization_27 (LN)     (None, 144, 64)     128      
 multi_head_attention_13 (MH)    (None, 144, 64)     66368    
 add_26 (Add)                   (None, 144, 64)      0        
 layer_normalization_28 (LN)     (None, 144, 64)     128      
 dense_31 (Dense)               (None, 144, 128)     8320     
 dropout_29 (Dropout)           (None, 144, 128)     0        
 dense_32 (Dense)               (None, 144, 64)      8256     
 dropout_30 (Dropout)           (None, 144, 64)      0        
 add_27 (Add)                   (None, 144, 64)      0        
 layer_normalization_29 (LN)     (None, 144, 64)     128      
 multi_head_attention_14 (MH)    (None, 144, 64)     66368    
 add_28 (Add)                   (None, 144, 64)      0        
 layer_normalization_30 (LN)     (None, 144, 64)     128      
 dense_33 (Dense)               (None, 144, 128)     8320     
 dropout_31 (Dropout)           (None, 144, 128)     0        
 dense_34 (Dense)               (None, 144, 64)      8256     
 dropout_32 (Dropout)           (None, 144, 64)      0        
 add_29 (Add)                   (None, 144, 64)      0        
 layer_normalization_31 (LN)     (None, 144, 64)     128      
 multi_head_attention_15 (MH)    (None, 144, 64)     66368    
 add_30 (Add)                   (None, 144, 64)      0        
 layer_normalization_32 (LN)     (None, 144, 64)     128      
 dense_35 (Dense)               (None, 144, 128)     8320     
 dropout_33 (Dropout)           (None, 144, 128)     0        
 dense_36 (Dense)               (None, 144, 64)      8256     
 dropout_34 (Dropout)           (None, 144, 64)      0        
 add_31 (Add)                   (None, 144, 64)      0        
 layer_normalization_33 (LN)     (None, 144, 64)     128      
 flatten_1 (Flatten)            (None, 9216)         0        
 dropout_35 (Dropout)           (None, 9216)         0        
 dense_37 (Dense)               (None, 2048)         18876416 
 dropout_36 (Dropout)           (None, 2048)         0        
 dense_38 (Dense)               (None, 1024)         2098176  
 dropout_37 (Dropout)           (None, 1024)         0        
 dense_39 (Dense)               (None, 10)           10250    
==============================================================

\end{Verbatim}

==> chapters/perm_imagenet.tex <==
Sushil Thapa (the "Researcher") has requested permission to use the ImageNet database (the "Database") at Princeton University and Stanford University. In exchange for such permission, the Researcher hereby agrees to the following terms and conditions:
\begin{enumerate}
    \item Researcher shall use the Database only for non-commercial research and educational purposes.
    \item Princeton University and Stanford University make no representations or warranties regarding the Database, including but not limited to warranties of non-infringement or fitness for a particular purpose.
    \item Researcher accepts full responsibility for his or her use of the Database and shall defend and indemnify the ImageNet team, Princeton University, and Stanford University, including their employees, Trustees, officers, and agents, against any and all claims arising from Researcher's use of the Data\-base, including but not limited to Researcher's use of any copies of copyrighted images that he or she may create from the Data\-base.
    \item Researcher may provide research associates and colleagues with access to the Database provided that they first agree to be bound by these terms and conditions.
    \item Princeton University and Stanford University reserve the right to terminate Researcher's access to the Database at any time.
    \item If Researcher is employed by a for-profit, commercial entity, Researcher's employer shall also be bound by these terms and conditions, and Researcher hereby represents that he or she is fully authorized to enter into this agreement on behalf of such employer.
    \item The law of the State of New Jersey shall apply to all disputes under this agreement.
\end{enumerate}

\newpage


